Fast Distributed Inference Serving for Large Language Models

Large language models (LLMs) power a new generation of interactive AI applications exemplified by ChatGPT. The interactive nature of these applications demands low latency for LLM inference. Existing LLM serving systems use run-to-completion processing for inference jobs, which suffers from head-of-line blocking and long latency. We present FastServe, a distributed inference serving system for LLMs. FastServe exploits the autoregressive pattern of LLM inference to enable preemption at the granularity of each output token. FastServe uses preemptive scheduling to minimize latency with a novel skip-join Multi-Level Feedback Queue scheduler. Based on the new semi-information-agnostic setting of LLM inference, the scheduler leverages the input length information to assign an appropriate initial queue for each arrival job to join. The higher priority queues than the joined queue are skipped to reduce demotions. We design an efficient GPU memory management mechanism that proactively offloads and uploads intermediate state between GPU memory and host memory for LLM inference. We build a system prototype of FastServe and experimental results show that compared to the state-of-the-art solution vLLM, FastServe improves the throughput by up to 31.4x and 17.9x under the same average and tail latency requirements, respectively.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}



==> sections/motivation.tex <==
\section{Motivation}

\iffalse
\begin{table*}[t]
    \begin{center}
        \begin{tabularx}{\textwidth}{lXXXl}
        \toprule
            & \centering\textbf{Low job completion time}
            & \centering\textbf{Efficient GPU memory usage}
            & \centering\textbf{Efficient distributed computation}
            &
            \\
        \midrule
            \textbf{FasterTransformer}
            & 
            & 
            & 
            &
            \\
        \textbf{Orca}~\cite{?}
            & 
            & \centering$\checkmark$
            & 
            &
            \\
        \textbf{Naive MLFQ}
            & \centering$\checkmark$
            & 
            & 
            & 
            \\
        \textbf{\sysname (ours)}
            & \centering$\checkmark$
            & \centering$\checkmark$
            & \centering$\checkmark$
            &
            \\
        \bottomrule
        \end{tabularx}
        \caption{Comparison between \sysname and existing LLM serving systems.}
        \label{table:motivation:system_properties}
    \end{center}
    \end{table*}
\fi

In this section, we first discuss the limitations of existing solutions for
inference serving of LLMs. Then we describe the opportunities and challenges.

\subsection{Limitations of Existing Solutions}

The current state-of-the-art solution of LLM serving system is Orca~\cite{?}.
Orca schedules execution at the granularity of iteration instead of job
based on the auto-regressive nature of LLMs. In this way, Orca can return
responses of early-finished jobs in a batch of jobs earlier, and can
batch unfinished jobs with late-join jobs. Orca also proposes selective
batching to batch an arbitrary set of jobs\todo{consistent to job or job}. As a result, Orca can achieve
higher throughput other LLM serving systems.

However, for interactive AI applications, users care about JCT of jobs
rather than the throughput of the LLM serving system. In terms of JCT, Orca
cannot provide good user experience, because it only uses a simple scheduling
algorithm, First Come First Serve (FCFS), which may cause head-of-line (HOL)
blocking and thus hurt user experience.

For example, when Orca is processing jobs with long input sequence length or
long output sequence length, subsequent jobs have to wait for the completion
in the job queue for a long time, because the LLM serving system can only
process limited job at a time. As a result, the JCT of Orca is not optimal.
The LLM serving system can execute shorter jobs first to achieve lower
average JCT.

As for GPU memory consumption, FCFS simplifies the memory management of Orca.
Orca only needs to allocate GPU memory for KV cache of jobs in the
processing and release them after completion. As a result, all allocated KV
caches are active for the LLM inference. The required GPU memory is minimal.
Therefore, the capacity of the LLM serving system is not bounded by the GPU
memory capacity.

Existing LLM serving systems also do not support distributed LLM inference well
enough. Although Orca can partition LLMs into multiple pieces with the same
number of parameters, the partitioning may still cause pipeline bubbles.
Figure~\ref{fig:motivation:heterogeneity} shows that the JCT of jobs to LLM
inference is varied under different input sequence length and output sequence
length. The JCT of a job can be XXX$\times$ longer than the JCT of another
job. Existing LLM serving systems treat all jobs equally. When different
jobs are processed in different pipeline stages, heterogeneity of jobs
creates the pipeline bubbles, which increase the JCT of subsequent jobs.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/time_vs_jobsize.png}
    \caption{JCT of jobs with different input sequence length and output sequence length. \todo{Only a placeholder, replace this figure with JCT vs. batch size.}}
    \label{fig:motivation:heterogeneity}
\end{figure}

In summary, The SOTA solution, Orca, is not suitable for interactive AI applications. As shown in Table~\ref{table:motivation:system_properties}, Orca is not distribution computation efficient and cannot provide low JCT for interactive applications.

% Simple FIFO scheduling, is not optimal in terms of JCT.

% \subsection{Oracle: SRPT}

\subsection{Opportunities and Challenges}

Because existing solutions presume run-to-completion scheduling, they cannot provide low JCT for interactive applications due to HOL blocking. Instead, the preemption mechanism can be used to improve the scheduling algorithm. Each job consists of multiple iterations. Each iteration generates one token of the response. When one iteration of a job finishes, the scheduler can preempt the job in the processing and schedule another job to execute. With the help of the preemption mechanism, the scheduler can schedule the job with the shortest remaining execution time (SRPT) to execute. The SRPT scheduling algorithm has been proofed as the optimal scheduling algorithm in terms of JCT~\cite{?}.

However, SRPT is not a practical solution for LLM serving systems. SRPT needs to know the remaining execution time of a job. Different from one-shot prediction tasks, such as image classification, LLM inference is an iterative process. The remaining execution time of a job is not known until the job finishes. The remaining execution of a job is also hard to be predicted, because it is determined by the semantics of a job. Therefore, the scheduler cannot schedule the job with the shortest remaining execution time to execute.

To approximate the optimal SRPT scheduling, a well-known approximate scheduling policy without prior knowledge is the Multi-Level Feedback Queue (MLFQ)~\cite{?} or Least Attained Service (LAS)~\cite{?}. The essence of MLFQ is to schedule the job with the shortest executed time. Ideally, in this way, a naive MLFQ scheduler can finish shorter jobs earlier than FCFS and thus achieves lower JCT.

Unfortunately, the naive MLFQ scheduler may consume huge GPU memory. For all preempted jobs in the pending state, the MLFQ scheduler still needs to keep the KV cache of the jobs in the GPU memory for the future token generation. Compared to FCFS, the naive MLFQ scheduler needs to allocate more GPU memory for these inactive KV caches. As mentioned before, this KV caches may even occupy more GPU memory than the model parameters of LLMs. Therefore, the limited GPU memory capacity may decrease the number of concurrent jobs that can be processed by the LLM serving system with the naive MLFQ policy compared to the FCFS policy, which increases the queueing delay of subsequent jobs and thus increases the JCT of jobs.

Last but not least, the naive MLFQ scheduler is based on the assumption that all iterations of jobs have the same execution time. However, as shown in Figure~\ref{fig:motivation:heterogeneity}, the execution time of iterations of jobs is varied. The naive MLFQ scheduler still cannot handle pipeline parallelism well.

In summary, as shown in Table~\ref{table:motivation:system_properties}, while the naive MLFQ scheduler can achieve lower JCT when having sufficient GPU memory, it still cannot efficiently use limited GPU memory and is not tailored for distributed LLM inference.

% As ChatGPT-like models are becoming popular, it is critical to provide high-performance LLM inference 
% for huge amount of user jobs. While current solutions like Orca which uses FCFS strategy have 
% optimized the serving systems for better throughput, the heterogeneous compute demand of token 
% generation leads these throughput-based serving systems into a sub-optimal state in terms of 
% user experience.

% Our targets:

% - interactive, optimize JCT => argue FCFS << SRPT

% - memory efficient

% - scability => reduce pipeline bubble

% \subsection{characteristics of autoregressive generation job}
% \label{subsec:characteristics}

% \begin{itemize}
% \item The job execution time is not fixed. It depends on both input length and output length. T = ax + b.
% In practice, the finish time is unpredictable.

% Figure: time vs. job size

% - X axis: output length

% - Y axis: JCT

% - Lines: different input length

% \item The iteration time is not fixed. (1) intra-job: first token takes more time, later tokens take almost the same time.
% (2) inter-job: the first iteration time depends on the input length. long-tailed distribution of input length: users usually
% ask questions less than 100 tokens, but some summarization task or long dialogues will have much longer input length.
% GPT-4 supports 32k input length in maximum. Maybe cite some papers in other areas.
% (3) inter-job: beam search can increase the iteration latency

% Figure: time vs. token index for different input length

% - X axis: index of the token

% - Y axis: time to generate the corresponding token

% - Lines: different input length

% Figure: time vs. token index for different beam size

% - X axis: index of the token

% - Y axis: time to generate the corresponding token

% - Lines: different beam size

% \item burstiness: common in any serving workload

% \end{itemize}

% \subsection{FIFO is bad under these characteristics}

% Prove FIFO is bad under some of these characteristics when target average JCT. Introduce SRPT here.

% % Figure: average JCT vs. long-tailed distribution of input length

% % - X axis: long-tailed extent

% % - Y axis: average JCT

% % - Lines: FCFS vs. SRPT

% % - Trend: down

% Figure: average JCT vs. output length

% - X axis: output length

% - Y axis: average JCT

% - Lines: FIFO vs. SRPT

% - Trend: down

% - Implication: FIFO is bad for Long-run job

% Figure: average token response time vs. burstiness

% - X axis: CV

% - Y axis: average JCT

% - Lines: FIFO vs. SRPT

% - Trend: down

% - Implication: FIFO is bad for bursty workload

% Prove SRPT is bad, because SRPT will increase the number of under-processing jobs which incurs larger GPU memory usage.

% Option 1
% - Y: max memory consumption (KV slot)
% - X: long tail or burstiness
% - Lines: FIFO vs. SRPT

% Option 2
% - Y: memory consumption (KV slot)
% - X: time
% - Lines: FIFO vs. SRPT


% \subsection{Heterogeneous compute demand induces Pipeline bubble}
% \S\ref{subsec:characteristics} shows that in a single job, the first token takes more time (intra-job heterogeneity), 
% and different jobs may have significantly different first iteration latency due to input length and later iteration latency
% due to beam width (iter-job heterogeneity).

% In practice, we use pipeline parallelism to serve bigger model, which will introduce pipeline bubble under heterogeneous jobs.

% Figure: average token response time vs. heterogeneity

% - X axis: the variance of input length

% - Y axis: average token response time

% - Lines: FIFO vs. SRPT

% - Trend: down



